Better Metrics for Ranking SE Researchers

This paper studies how SE researchers are ranked using a variety of metrics and data from 35,406 authors of 35,391 papers from 34 top SE venues in the period 1992-2016. Based on that analysis, we: deprecate the widely used "h-index", favoring instead an alternate Weighted Page Rank(PR_W) metric that is somewhat analogous to the PageRank(PR) metric developed at Google. Unlike the h-index, PR_W rewards not just citation counts but also how often authors collaborate. Using PR_W, we offer a ranking of the top 20 SE authors in the last decade.

==> damp_pr.tex <==
\begin{mdframed}

{\centering
\includegraphics[scale=0.45]{figs/png_damp_naive.png}
\vspace*{-8mm}
\captionof{figure}{\label{fig:damp_pr}Scores of top 20 authors using \textbf{h-index weighted Page Rank} when $\theta$ is varied from 0 to 1 in intervals of 0.05}
\par}



The figures above represent the ranks of the top 20 authors using \textbf{PR}, \textbf{PR$_\text{publ}$} and \textbf{PR$_\text{cite}$} with the values of $\theta$ from \eref{pr} and \eref{pr_w} varied between 0 and 1 at intervals of 0.5. We can see that the relative ordering of the ranks look almost same. We can observe small changes at lower values(< 0.15) of $\theta$ but at later values the ranks are almost similar. The authors of PageRank, Page \etal in their paper justifies this that the optimum value of $\theta$ help the algorithm converge faster. This is because PageRank is essentially a markov chain algorithm trying to stabilize all the nodes(in this case authors) of the graph. In this paper we use $\theta = 0.5$, to allocate equal weight to both parts of page rank.
\end{mdframed}


==> dependencies.tex <==
\RequirePackage{xcolor}
\ifCLASSOPTIONcompsoc
  % The IEEE Computer Society needs nocompress option
  % requires cite.sty v4.0 or later (November 2003)
  \usepackage[nocompress]{cite}
\else
  % normal IEEE
  \usepackage{cite}
\fi
\usepackage{array}
\usepackage{lineno,hyperref}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{balance}
\usepackage{flushend}
% \usepackage{natbib}
\usepackage{color} 
\usepackage{graphics} 
% \usepackage{cite}
\usepackage{rotating}
\usepackage{eqparbox}
\usepackage{graphics}
\usepackage{colortbl}
\usepackage{wrapfig}
\usepackage{times}
%\usepackage{mathptmx} \usepackage[scaled=.90]{helvet} \usepackage{courier}
% \usepackage{balance}
\usepackage{flushend}
\usepackage{picture}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage[export]{adjustbox}
\usepackage{amsmath}
\usepackage{listings}
\usepackage{mdframed}
\usepackage{algorithm,algorithmicx}
\usepackage{algpseudocode}
\usepackage{wrapfig}
\usepackage{caption}

\usepackage{rotating}
\definecolor{Gray}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\definecolor{Blue}{RGB}{0,29,193}
\definecolor{rc1}{RGB}{253,237,236}
\definecolor{rc2}{RGB}{218,247,166}
\definecolor{rc3}{RGB}{174,214,241}
\definecolor{rc4}{RGB}{242,244,244}
\definecolor{rc5}{RGB}{255,195,0}
\definecolor{rc6}{RGB}{199,0,57}
\definecolor{rc7}{RGB}{144,12,63}

\renewcommand{\footnotesize}{\scriptsize}
\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgray}{gray}{0.6}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%%% graph
\newcommand{\crule}[3][darkgray]{\textcolor{#1}{\rule{#2}{#3}}}
\definecolor{Gray}{gray}{0.95}
\definecolor{LightGray}{gray}{0.975}

%% timm tricks
\newcommand{\eref}[1]{Eq.~\ref{eq:#1}}
\newcommand{\fref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tref}[1]{Table~\ref{tab:#1}}
\newcommand{\boldm}[1]{$\bm{#1}$}
\newcommand{\bit}[1]{\textbf{\textit{#1}}}
\newcommand{\bi}{\begin{itemize}[leftmargin=0.4cm]}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\tion}[1]{\S\ref{sect:#1}}
\newcommand{\fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\tab}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{Equation~\ref{eq:#1}}
\newcommand{\PM}{$\pm$}
\newcommand{\desc}[1] {
    \medskip
    \raggedright
    \small
    #1
}
\newcommand{\bcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\etal}{et. al. }
%% space saving measures
\let\labelindent\relax
\usepackage[shortlabels]{enumitem}  
\usepackage{url}

\usepackage{graphicx}
\usepackage{multirow}
% \usepackage[svgnames]{xcolor}
% \usepackage[table, svgnames]{xcolor}
\usepackage[framed]{ntheorem}
\usepackage{framed}
\usepackage{tikz}
\usetikzlibrary{shadows}
%\newtheorem{Lesson}{Lesson}
\theoremclass{Lesson}
\theoremstyle{break}

% inner sep=10pt,
\tikzstyle{thmbox} = [rectangle, rounded corners, draw=black,
  fill=Gray!20,  drop shadow={fill=black, opacity=1}]
\newcommand\thmbox[1]{%
  \noindent\begin{tikzpicture}%
  \node [thmbox] (box){%
\begin{minipage}{.9\textwidth}%    
      \vspace{-3mm}#1\vspace{-3mm}%
    \end{minipage}%
  };%
  \end{tikzpicture}}

\let\theoremframecommand\thmbox
\newshadedtheorem{lesson}{Result}

\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\newcommand{\mc}[2]{\multicolumn{#1}{|c|}{#2}}
\newcommand{\h}{\hspace{17pt}}
\newcommand{\hh}{\hspace{35pt}}
\newcommand{\rA}{\cellcolor{rc1}}
\newcommand{\rB}{\cellcolor{rc2}}
\newcommand{\rC}{\cellcolor{rc3}}
\newcommand{\rD}{\cellcolor{rc4}}
\newcommand{\rE}{\cellcolor{rc5}}
\newcommand{\rF}{\cellcolor{rc6}}
\newcommand{\legend}[2]{\colorbox{#1}{\makebox(9,3){}} #2}
